Deep Dependency Networks for Multi-Label Classification

We propose a simple approach which combines the strengths of probabilistic graphical models and deep learning architectures for solving the multi-label classification task, focusing specifically on image and video data. First, we show that the performance of previous approaches that combine Markov Random Fields with neural networks can be modestly improved by leveraging more powerful methods such as iterative join graph propagation, integer linear programming, and $\ell_1$ regularization-based structure learning. Then we propose a new modeling framework called deep dependency networks, which augments a dependency network, a model that is easy to train and learns more accurate dependencies but is limited to Gibbs sampling for inference, to the output layer of a neural network. We show that despite its simplicity, jointly learning this new architecture yields significant improvements in performance over the baseline neural network. In particular, our experimental evaluation on three video activity classification datasets: Charades, Textually Annotated Cooking Scenes (TACoS), and Wetlab, and three multi-label image classification datasets: MS-COCO, PASCAL VOC, and NUS-WIDE show that deep dependency networks are almost always superior to pure neural architectures that do not use dependency networks.

==> content/4-model.tex <==
\subsection{Inputs to the PGM}
The output of the classification layer will be treated as the features extracted from the Convolutional Neural Network; thus, the size of this feature vector will be (1, number of true labels) for each instance. 
%The reason behind this is that it helps us model the relationships between these labels and the labels that the PGM will predict.
By using these features we fulfill two tasks at once. Firstly we can utilize the information extracted by the NNs and also model the relationships between the true labels and the output probabilities of the CNN. For example high feature probability for an activity open cupboard can help the model to interpret that it can be either open cupboard or close cupboard, since both these labels have similar kind of examples in the video. These relationships can be learned by PGMs and thus help in improving the model performance. 
In addition to this information, we can also use the inter-label dependencies to predict the final output. 
Thus the nodes in the PGMs will be of two types - $\displaystyle \rve$ and $\displaystyle \rvy$. The nodes $\displaystyle \rvy$ will correspond to the output labels that will be inferred from the PGM. Furthermore, $\displaystyle \rve$ nodes will represent the evidence we get from the CNN. Thus we will define a PGM over the graph $\displaystyle \gG$ whose nodes will be  $\displaystyle \sX = (y_1,....., y_n, x_1,.....,x_n)$ where n is the total number of labels in the given dataset. 


\subsection{Markov Random Fields}
\subsubsection{Structure Learning}
We will define a joint distribution over all the variables in $\displaystyle \rvy$ and $\displaystyle \rve$. For each node $\displaystyle y_i$ its neighbors will be ($\displaystyle \sN(y_i), x_i$). Where $\displaystyle \sN(y_i) \subseteq (y_1, ..... , y_{i-1}, y_{i+1}, ...... , y_{n})$. For structure learning of the MRF we will use $\displaystyle L_1$-regularized logistic regression \citep{NIPS2006_86b20716, NIPS2006_a4380923}, to get the set $\sN(y_i)$ for each $\displaystyle y_i$. $\displaystyle \sN(y_i)$ is also called Markov blanket of the node $y_i$. We have provided an example of how the MRF would look in Figure \ref{fig:pgm_lr_dn} where $\displaystyle \sN(y_1) = y_2, \sN(y_2) = (y_1, y_3), \sN(y_3) = y_2 $. This method helps us find the set of nodes highly related to the given node to create the neighborhood and thus include important relationships in the graph. The only issue with MRFs is that we need to bound the number of neighbors for each node in the graph; otherwise, if the graph is too densely connected, inference tasks in MRFs become hard for exact inference. Approximate inference techniques also become less accurate, thus getting poorer results. Thus for these experiments, we learn MRFs with neighborhood size capped by 10. 

\subsubsection{Parameter Learning}
We learn the parameters of the MRF by using Maximum Pseudo-likelihood Parameter Estimation \cite{koller2009probabilistic}. We do not use Likelihood Parameter Estimation because it requires running inference over the network in each iteration, making the learning process very slow. However, that is not the case if we use Pseudo-likelihood as the training objective. Furthermore, the inference becomes even slower if the model has a high tree width. We use L2 regularization with stochastic gradient descent to learn the parameters of the MRF so that the model does not over-fit the data. In many cases, pseudo-likelihood as an objective can perform very well, reducing the computational cost of learning. Pseudo-likelihood can be defined as follows
\begin{equation}
\displaystyle l_{P L}(\theta: \mathcal{D})=\frac{1}{M} \sum_{m=1}^M \sum_{j=1}^n \ln p \left(x_{j}[m] \mid x_{-j}[m], \boldsymbol{\theta}\right)
\end{equation}
where $\displaystyle \theta$ is the model's parameters, $\displaystyle M$ is the number of examples in dataset $\displaystyle \mathcal{D}$, and $\displaystyle n$ is the number of variables in the model. 

\subsubsection{Inference}
We will perform two different tasks for inference, maximum a posteriori (MAP) estimation task using Integer Linear Programming solver and Belief Update task using Iterative Join-Graph Propagation (IJGP) solver. MAP inference can be defined as assigning the most probable values to the variables in a graph, given the evidence. Finding the MAP assignment is an NP-hard task unless we are given tree-structured graphs or graphs with bounded tree-width \citep{dechter2003constraint, globersonFixingMaxProductConvergent}. Belief Update is the task where we compute the posterior probability $\displaystyle P(Y|e)$ where $\displaystyle Y$ are the query nodes, and $e$ is the given evidence. IJGP is an iterative version of join-tree clustering that can be used as a generalized belief propagation method. Thus we are performing two tasks, one that provides us with the assignment to the variables and one that outputs the probabilities of the query nodes given the evidence. These two sophisticated inference techniques for MRFs perform well for the corresponding tasks.  


\subsection{Conditional Dependency Networks}

\yu{We need to present Deep Dependency Networks in the method section.}

\subsubsection{Structure Learning}
We will use the conditional dependency networks proposed in \citep{guo2011multi} that have been proved to model the inter-label dependencies for the multi-label classification task. For this model, we will define a conditional joint distribution over all the variables in $\displaystyle \rvy$, assuming that the evidence variables $\displaystyle \rve$ are given, and this evidence comes from CNN. For each node $\displaystyle y_i$ its parent set will be $\displaystyle \parents_\gG(y_i) = \{y_{-i}, x\}$ and the distribution $\displaystyle \gP$ will be defined only on the $\displaystyle \rvy$ variables, being conditioned on $\displaystyle \rve$. By doing this, we will get a model where the Markov blanket (MB) of each node will be all the other label nodes($\displaystyle y_{-i}$) and all the feature nodes ($\displaystyle \rve$). We have provided an example of how the DN would look in Figure \ref{fig:pgm_lr_dn}. We use two models to define the conditional probability distributions in $\displaystyle \gP$; the first is a logistic regression (LR) model. Representing dependency networks using logistic regression was proposed in \citet{heckerman2000dependency}. Since Neural Networks have been proved to have more representation power than the Logistic Regression model, we will also represent each distribution using a NN. 

\subsubsection{Parameter Learning}
For both the models, we will learn the parameters by minimizing the Cross-Entropy loss on the output variable of the model, using stochastic gradient descent. For the logistic regression model, we use L1 regularization to learn the Markov blanket of the node and thus only choose nodes that help predict the output node. We use regularization for both models to stop them from overfitting. While training, the input to the model that predicts $\displaystyle y_{i}$ will be a vector that is the concatenation of $\displaystyle y_{-i}$ and $\displaystyle x$, and we will have n of these models, each for a $\displaystyle y_{i}$. Since each of the models representing the distribution of a different $\displaystyle y_{i}$ are not dependent on each other, we can train them in parallel, thus making the learning process very fast. We also implemented both the models in PyTorch, which helps us to use GPUs while training making it even faster. 


\subsubsection{Inference}
We will use a Systematic-Scan Gibbs Sampling to perform the inference for Dependency Networks. There is a possibility that Dependency Networks may not model a probability distribution. However, \citet{heckerman2000dependency} has argued that if the number of samples is large enough during inference, then the distribution of the outputs provided by the Gibbs sampler is consistent with a conditional distribution. Since cycles are also allowed in Dependency Networks, we cannot use inference methods that can be used with Bayesian Networks and Markov Networks, like Variable Elimination and  Iterative Joint Graph Propagation. 



To estimate the marginal probabilities of the output variable, we will use \textbf{Mixture Estimator}, which is defined in \ref{Mixture_Estimator}
$$
\label{Mixture_Estimator}
\displaystyle \hat{P}\left(x_{i}\right)=\frac{1}{N} \sum_{j=1}^{N} P\left(x_{i}^{(j)} \mid \textbf{x}_{MB(X_{i})}^{(j)}\right)
$$
where $\displaystyle x_i$ is the node for which we want to find the probabilities and $\displaystyle \textbf{x}_{MB(x_{i})}$ is the Markov blanket of the variable $\displaystyle x_i$. The variable $\displaystyle j$ goes over the examples. 
\begin{figure}
    \begin{subfigure}{.49\textwidth}
        \centering
        \includegraphics[width= 0.98\textwidth]{icml2023/images/dn.pdf}
        \caption{Dependency Network Structure}
    \end{subfigure}\hfill
    \begin{subfigure}{.49\textwidth}
        \centering
        \includegraphics[width= 0.98\textwidth]{icml2022/images/mrf.pdf}
        \caption{Markov Random Field Structure}
    \end{subfigure}
    \caption{Probabilistic Graphical Models}
    \label{fig:pgm_lr_dn}
\end{figure}

% \begin{frame}
% \frametitle{Systematic-Scan Gibbs Sampler}
% The Systematic-Scan Gibbs Sampler algorithm is given by\\
% \begin{enumerate}
%     \item Sample s = Random assignment to $\forall X_i$ nodes. \\
%     \textbf{Iterate till convergence or fixed number of iterations:}
% \\
% For iteration t+1
% \\
% For all i = 1,....,n 
%      \begin{enumerate}
%             \item Sample $(X_i^{(t+1)} = x_i)$ from $P(X_{i} \mid x_{1}^{(t+1)},...,x_{i-1}^{(t+1)},x_{i+1}^{t},...,x_{n}^{t},e_{1}^{(t+1)},...,e_{n}^{(t+1)})$
%             \item Replace $(X_i = x_i)$ in Sample s
%         \end{enumerate}
% \end{enumerate}
% \end{frame}
% \begin{frame}


\eat{The Systematic-Scan Gibbs Sampler algorithm can be performed as given in Algorithm \ref{alg:gibbs_alg}
\begin{algorithm}
\caption{Systematic-Scan Gibbs Sampling}
\begin{algorithmic}
\Procedure{Gibbs Sampling}{$s, num\_iter$} 
\Comment{Sample s = Random assignment to $\forall X_i$ nodes.}
\State $t \gets 0$
\While{$t \leq num\_iter$}
\State $t \gets t + 1$
\State $i \gets 0$
% For iteration t+1
\While{$i \leq n$}
            \State $t \gets t + 1$
            \State Sample $(Y_i^{(t)} = Y_i)$ from $P(y_{i} \mid y_{1}^{(t)},..,y_{i-1}^{(t)},y_{i+1}^{t-1},..,y_{n}^{t-1},e_{1}^{(t)},..,e_{n}^{(t)})$
            \State Replace $(Y_i = y_i)$ in Sample s
\EndWhile
\EndWhile
\EndProcedure
\end{algorithmic}
\label{alg:gibbs_alg}
\end{algorithm}}

% WHY WE DO NOT USE GNNs TO MODEL LABEL DEPENDENCIES



==> content/5-Joint-learning.tex <==
\yu{Joint training is only for DN right? This section looks like for both MRF and DN.}

To do joint training, we need to select appropriate loss functions defined over the parameters of all the corresponding models and then perform gradient descent to minimize this loss. We use two losses to train the joint model \textemdash the first loss function is the Binary Cross Entropy ($\displaystyle BCE_{cnn}$) loss applied to the outputs of the CNN and true labels. The second loss function is the same as before; however, it is applied to the outputs of all the models representing the conditional probability distributions of the DNs. The loss ($\displaystyle BCE_{dn}$) will be applied to the output predicted by the $i^{th}$ model in the dependency network, $\displaystyle \hat{y_i}$ and the  $i^{th}$ true label $\displaystyle \vy_i$. Thus for the joint model, we will have $(N+1)$ losses where N is the total number of true labels in the given dataset. 

To start the end-to-end training process, we perform the forward pass on the CNN by providing the clip/frame input. After the getting the outputs of the CNN, we can calculate $\displaystyle BCE_{cnn}(\hat{Y}, Y_{cnn})$. Moreover, since we already have the values of the final layer of the CNN, we can now do the forward pass for the DN. Then we calculate $\displaystyle BCE_{dn}(\hat{Y}_{(i)}, Y_{dn^{(i)}})$ for each model of the DN. The loss $\displaystyle L_{joint}$, given in equation \ref{eq:cnn_joint_loss} is the resulting joint objective function, and it will be used to update the parameters of the two models using stochastic gradient descent. We do the same things for both the DN models, NN and LR; the only thing that changes is how we calculate the $\displaystyle BCE_{dn}^{(i)}$ and back-propagate its gradient through the models. 

\begin{equation}
\label{eq:cnn_joint_loss}
L_{joint} = BCE_{cnn}\left( \hat{Y}, Y_{cnn}\right) + \frac{1}{N} \sum_{i=1}^{N} BCE_{dn}\left( \hat{Y}_{(i)}, Y_{dn^{(i)}}\right)
\end{equation}

For the proposed model, the number of conditional distributions in the dependency networks depends on the number of true labels in the classes. This can become an enormous overhead over the feature extractor for datasets with an enormous number of labels (activities) since this model will require too much GPU memory if we try to run all the models in parallel. Thus to alleviate this problem, we optimize the joint loss by only allowing a fixed number of DN forward and backward passes simultaneously. Furthermore, the number of concurrent passes can be increased if required. We make this work by storing the gradients corresponding to the outputs of the NN until all the passes are finished, and then we can back-propagate the gradients through the NN. After training the model, the inference process remains the same as the previously mentioned pipeline model. Thus this joint learning process only adds overhead while training and provides with moderate to good improvements in the model performance. 

\begin{figure}[h]
\begin{center}
%\framebox[4.0in]{$\;$}
\includegraphics[width=\textwidth]{icml2022/images/joint_back_prop.pdf}
\caption{Illustration of the joint learning process. Blue arrows represent forward pass. Red arrows represent backward pass}
\end{center}
\end{figure}

\eat{Now we will look at how to train the Dependency Network and CNN jointly. Firstly, we have two losses for the joint model; the first is Binary Cross Entropy ($\displaystyle BCE_{cnn}$) loss which is applied to the outputs of the CNN and true labels. The second loss ($\displaystyle BCE_{dn}$) is also the Cross-Entropy loss. However, it is applied to the outputs of all the Dependency Networks and their corresponding true labels separately. Thus for a network predicting $\displaystyle y_i$ the loss ($\displaystyle BCE_{dn}^{(i)}$) will be applied to the predicted output $\displaystyle \hat{y_i}$ and the true label $\displaystyle \vy_i$.} 

\eat{For the training iteration, we first do the forward pass on CNN by providing the clip/frame as input. After the forward pass through the CNN, we can calculate $\displaystyle BCE_{cnn}$. Moreover, since we already have the values of the final layer of the CNN, we can now do the forward pass for the DN by providing the concatenation of the true labels and outputs of the CNN as the input. Then we calculate $\displaystyle BCE_{dn}$ for all the DNs and back-propagate the gradients. To get the gradients for the CNN, we will first take the average of all the losses of the DNs ($\displaystyle \frac{1}{n} \sum_{i=1}^n BCE_{dn}^{(i)}$) and then add it to $\displaystyle BCE_{cnn}$. Since the inputs of the DNs are the outputs of the final layer of the CNN, the CNN and DN will be connected, and thus the loss corresponding to the DNs also depends on the variables in the CNN. Finally, these gradients are back-propagated through CNN. Thus the both the models are learned jointly and it helps to improve the performance over the pipeline model. }


==> content/9-future-work.tex <==
\eat{As we have mentioned before for some cases dependency networks might not correspond to valid distributions. Thus we cannot use more sophisticated inference techniques, that have been proposed for other probabilistic models, on dependency networks. But as we saw in this paper, learning better representations can be better than using more extensive inference techniques. What if we can use these sophisticated inference techniques on model that has a high representative power as well? Thus we will try to create a model which merges the advantages of both, MRFs and DNs to get even better results. There have been work that converted inconsistent dependency networks to markov networks \citep{lowdClosedFormLearningMarkov2012a}. Since we already have the better learned model, we can try to convert it to a different type of model for which, learning is hard but inference is fast and superior than dependency networks. }


\eat{
Sometimes dependency networks do not have valid distributions, but MRFs always correspond to a valid distribution. We will try to propose models which can take the advantages of both the models, the better representations from the DNs and better inference techniques from the MRFs. We can do the same by converting the better representations that we learn, to models on which we can do more sophisticated inferences. There have been work that converted dependency networks to markov networks \citep{lowdClosedFormLearningMarkov2012a}. }

==> content/notes.tex <==
Reasons:

IJGP versus ILP on JI and SA
1. IJGP helps in JI and SA but more on JI than SA
2. ILP helps more on SA but less on JI

IJGP versus ILP on MAP and LRAP
ILP is worse; IJGP may help in LRAP but loses on MAP consistently

SA: the set of labels predicted for a sample must exactly match the corresponding set of labels in y\_true.
JI: the size of the intersection divided by the size of the union of two label sets
mAP: 

max-marginal: --> JI 111 --->101 
MAP inference --> SA 111 --->101 . When not correct, it tends to produce too many labels which drives jaccard index low, but it is correct in more examples than IJGP.

Conclusion: Metrics which use discrete labels such as JI and SA

Dependency networks

Good points:
Accurate estimates of posterior probability
No sparsity constraint
implementation on GPUs and easy extensions for pytorch, tensorflow, embarassingly parallel

Bad points:
No consistent probability distribution; although given an ordering for Gibbs sampling, it converges. But for most practical problems, the distribution will be close to consistent. (Empirical distribution is always consistent and therefore if we had used the empirical distribution, we would always get a consistent dependency network).

Gibbs sampling is one of the only inference methods (mean-field inference, Lowd)but the performance is same. More advanced methods like IJGP are not available for dependency networks
----------------

We focus on the following multi-label action classification task: given a video partitioned into (continuous) segments and a pre-defined set of actions, label each segment with a subset of actions from the pre-defined set that are performed in the segment. We consider a simple version of this task where each action is a verb-noun pair. This task is a special case of the standard multi-label classification (MLC) task where given a pre-defined set of labels and a test example, the goal is to (learn a function from training data which will) assign each test example to a subset of labels from the pre-defined set.

It is well known that MLC is notoriously difficult because in practice the labels are often correlated and thus predicting them independently may lead to significant errors. Therefore, most advanced methods often explicitly model the relationship/dependencies between the labels either using probabilistic \citet{wang2008generative,rossiProceedingsTwentyThirdInternational2013b,Tan_2015_CVPR,pmlr-v52-dimauro16,wangEnhancingMultilabelClassification2014a,antonucci2013ensemble} or non-probabilistic methods \citet{papagiannopoulouDiscoveringExploitingDeterministic2015a, kongMultilabelClassificationMining2013a,wang2021semi,nguyenModularGraphTransformer2021,wangNovelReasoningMechanism2021a}. Intuitively, the same logic, modeling relationship between the labels (as well as the features), applies to multi-label action classification in videos. To this end, the primary goal of this paper is to develop a simple, general-purpose scheme that explicitly models the relationships between the labels using probabilistic representations and reasoning methods and works on top of neural feature extractors in order to improve the generalization accuracy.

Our work is inspired by previous work on hybrid models that combine probabilistic graphical models (PGMs) with neural networks (NNs) under the assumption that their strengths are often complementary (see for example \citet{johnson,krishan}); neural networks perform feature extractions and PGMs model the relationships between the labels and the features. In particular, these hybrid models have been used for solving a range of computer vision tasks such as image crowd counting \citep{hanImageCrowdCounting2017}, structured output prediction \citep{pmlr-doNeuralConditionalRandom2010}, visual relationship detection \citep{yuProbabilisticGraphicalModel_2022_CVPR}, modeling for epileptic seizure detection in multichannel EEG \citep{craleyIntegratingConvolutionalNeural2019a}, phonetic recognition \citep{morrisConditionalRandomFields2008}, Face Sketch Synthesis \citep{zhangNeuralProbabilisticGraphical2020}, semantic image segmentation \citep{chenDeepLabSemanticImage2018, linEfficientPiecewiseTraining2015}, animal pose tracking \citep{wuDeepGraphPoseNEURIPS2020}, pose estimation \citep{chenArticulatedPoseEstimation2014} and Adaptive Team Training \cite{rollArtificialIntelligenceEducation2021}. In this paper, we seek to extend these previously proposed approaches for solving the multi-label action classification task in video.

As a starting point, we investigated using Markov random fields (or Markov networks), which are a type of undirected graphical model to capture the relationship between the features computed using convolutional neural networks and the labels. Unlike previous work which used these MRF/CRF+CNN hybrids, our goal was to evaluate whether advanced reasoning and learning approaches such as iterative join graph propagation (a type of generalization Belief propagation technuque), integer linear programming based techniques for computing most probable explanations and l1-regularization based structure learning methods improve the accuracy on the test set. We used several metrics such as mean average precision, label ranking average precision, subset accuracy and jaccard index, and three datasets: Charades, TACoS and Wetlab. We found that the advanced methods typically improve the jaccard index and subset accuracy but do not improve over the baseline neural models on the other two metrics.

We speculated that the primary reason for lack of substantial improvement (when MRFs are used) is the sparsity constraint which enables fast, accurate inference but often yields models that do not generalize well on high-dimensional data. To circumvent this problem, we propose to use dependency networks, a class of models that admits fast, accurate learning but no advanced reasoning methods


% Our first approach points:
(1) Markov random fields are used to model relationship between features and labels. Our goal was to test whether advanced reasoning and learning approaches such as generalized belief propagation, advanced MAP inference techniques based on integer linear programming and l1-regularization based structure learning improve the performance. In our experiments on 3 datasets, we observed modest to no improvement in generalization performance using these methods. We speculated that the primary reason for lack of substantial improvement is the sparsity constraint which enables fast, accurate inference but often yields models that do not generalize well.

To circumvent this problem, we propose to use dependency networks. Learning is easy and efficient in these networks; although inference is only via Gibbs sampling.


% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% % I. Computer Vision Tasks using Transformers and CNNs
% % I1. Semantic Segmentation

%   copyright = {arXiv.org perpetual, non-exclusive license}
% }

% @article{Liu2021PolarizedST,
%   title={Polarized Self-Attention: Towards High-quality Pixel-wise Regression},
%   author={Huajun Liu and Fuqiang Liu and Xinyi Fan and Dong Huang},
%   journal={ArXiv},
%   year={2021},
%   volume={abs/2107.00782}
% }

% @InProceedings{Girdhar_2022_CVPR,
%     author    = {Girdhar, Rohit and Singh, Mannat and Ravi, Nikhila and van der Maaten, Laurens and Joulin, Armand and Misra, Ishan},
%     title     = {Omnivore: A Single Model for Many Visual Modalities},
%     booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
%     month     = {June},
%     year      = {2022},
%     pages     = {16102-16112}
% }

% @article{duta2020pyramidal,
%   title={Pyramidal convolution: rethinking convolutional neural networks for visual recognition},
%   author={Duta, Ionut Cosmin and Liu, Li and Zhu, Fan and Shao, Ling},
%   journal={arXiv preprint arXiv:2006.11538},
%   year={2020}
% }



% % I2. Image Classification
% @inproceedings{brock2021high,
%   title={High-performance large-scale image recognition without normalization},
%   author={Brock, Andy and De, Soham and Smith, Samuel L and Simonyan, Karen},
%   booktitle={International Conference on Machine Learning},
%   pages={1059--1071},
%   year={2021},
%   organization={PMLR}
% }

% @InProceedings{Liu_2022_CVPR,
%     author    = {Liu, Zhuang and Mao, Hanzi and Wu, Chao-Yuan and Feichtenhofer, Christoph and Darrell, Trevor and Xie, Saining},
%     title     = {A ConvNet for the 2020s},
%     booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
%     month     = {June},
%     year      = {2022},
%     pages     = {11976-11986}
% }

% @inproceedings{NIPS2012_c399862d,
%  author = {Krizhevsky, Alex and Sutskever, Ilya and Hinton, Geoffrey E},
%  booktitle = {Advances in Neural Information Processing Systems},
%  editor = {F. Pereira and C.J. Burges and L. Bottou and K.Q. Weinberger},
%  pages = {},
%  publisher = {Curran Associates, Inc.},
%  title = {ImageNet Classification with Deep Convolutional Neural Networks},
%  url = {https://proceedings.neurips.cc/paper/2012/file/c399862d3b9d6b76c8436e924a68c45b-Paper.pdf},
%  volume = {25},
%  year = {2012}
% }

% @inproceedings{DBLP:journals/corr/SimonyanZ14a,
%   author    = {Karen Simonyan and
%               Andrew Zisserman},
%   editor    = {Yoshua Bengio and
%               Yann LeCun},
%   title     = {Very Deep Convolutional Networks for Large-Scale Image Recognition},
%   booktitle = {3rd International Conference on Learning Representations, {ICLR} 2015,
%               San Diego, CA, USA, May 7-9, 2015, Conference Track Proceedings},
%   year      = {2015},
%   url       = {http://arxiv.org/abs/1409.1556},
%   timestamp = {Wed, 17 Jul 2019 10:40:54 +0200},
%   biburl    = {https://dblp.org/rec/journals/corr/SimonyanZ14a.bib},
%   bibsource = {dblp computer science bibliography, https://dblp.org}
% }

% @misc{https://doi.org/10.48550/arxiv.2010.11929,
%   doi = {10.48550/ARXIV.2010.11929},
  
%   url = {https://arxiv.org/abs/2010.11929},
  
%   author = {Dosovitskiy, Alexey and Beyer, Lucas and Kolesnikov, Alexander and Weissenborn, Dirk and Zhai, Xiaohua and Unterthiner, Thomas and Dehghani, Mostafa and Minderer, Matthias and Heigold, Georg and Gelly, Sylvain and Uszkoreit, Jakob and Houlsby, Neil},
  
%   keywords = {Computer Vision and Pattern Recognition (cs.CV), Artificial Intelligence (cs.AI), Machine Learning (cs.LG), FOS: Computer and information sciences, FOS: Computer and information sciences},
  
%   title = {An Image is Worth 16x16 Words: Transformers for Image Recognition at Scale},
  
%   publisher = {arXiv},
  
%   year = {2020},
  
%   copyright = {arXiv.org perpetual, non-exclusive license}
% }


% % I3. Pose Estimation
% @InProceedings{Reddy_2021_CVPR,
%     author    = {Reddy, N Dinesh and Guigues, Laurent and Pishchulin, Leonid and Eledath, Jayan and Narasimhan, Srinivasa G.},
%     title     = {TesseTrack: End-to-End Learnable Multi-Person Articulated 3D Pose Tracking},
%     booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
%     month     = {June},
%     year      = {2021},
%     pages     = {15190-15200}
% }

% @article{bazarevsky2020blazepose,
%   title={Blazepose: On-device real-time body pose tracking},
%   author={Bazarevsky, Valentin and Grishchenko, Ivan and Raveendran, Karthik and Zhu, Tyler and Zhang, Fan and Grundmann, Matthias},
%   journal={arXiv preprint arXiv:2006.10204},
%   year={2020}
% }

% % I4. Object Detection
% @InProceedings{Liu_2022_CVPR,
%     author    = {Liu, Ze and Hu, Han and Lin, Yutong and Yao, Zhuliang and Xie, Zhenda and Wei, Yixuan and Ning, Jia and Cao, Yue and Zhang, Zheng and Dong, Li and Wei, Furu and Guo, Baining},
%     title     = {Swin Transformer V2: Scaling Up Capacity and Resolution},
%     booktitle = {Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
%     month     = {June},
%     year      = {2022},
%     pages     = {12009-12019}
% }

% @inproceedings{redmon2016you,
%   title={You only look once: Unified, real-time object detection},
%   author={Redmon, Joseph and Divvala, Santosh and Girshick, Ross and Farhadi, Ali},
%   booktitle={Proceedings of the IEEE conference on computer vision and pattern recognition},
%   pages={779--788},
%   year={2016}
% }


% % I6. Image Synthesis
% @inproceedings{ramesh2021zero,
%   title={Zero-shot text-to-image generation},
%   author={Ramesh, Aditya and Pavlov, Mikhail and Goh, Gabriel and Gray, Scott and Voss, Chelsea and Radford, Alec and Chen, Mark and Sutskever, Ilya},
%   booktitle={International Conference on Machine Learning},
%   pages={8821--8831},
%   year={2021},
%   organization={PMLR}
% }

% @misc{esser2020taming,
%       title={Taming Transformers for High-Resolution Image Synthesis},
%       author={Patrick Esser and Robin Rombach and Björn Ommer},
%       year={2020},
%       eprint={2012.09841},
%       archivePrefix={arXiv},
%       primaryClass={cs.CV}
% }

==> misc/authors.tex <==
\author{Antiquus S.~Hippocampus, Natalia Cerebro \& Amelie P. Amygdale \thanks{ Use footnote for providing further information
about author (webpage, alternative address)---\emph{not} for acknowledging
funding agencies.  Funding acknowledgements go at the end of the paper.} \\
Department of Computer Science\\
Cranberry-Lemon University\\
Pittsburgh, PA 15213, USA \\
\texttt{\{hippo,brain,jen\}@cs.cranberry-lemon.edu} \\
\And
Ji Q. Ren \& Yevgeny LeNet \\
Department of Computational Neuroscience \\
University of the Witwatersrand \\
Joburg, South Africa \\
\texttt{\{robot,net\}@wits.ac.za} \\
\AND
Coauthor \\
Affiliation \\
Address \\
\texttt{email}
}

==> misc/keywords.tex <==
% Keywords. The author(s) should pick words that accurately describe the work being
% presented. Separate the keywords with commas.
\keywords{probabilistic graphical models, action classification,  multi-label classification, combining probabilistic models with deep learning, end-to-end learning}
